Preconditioned infinite GMRES for parameterized linear systems

We are interested in obtaining approximate solutions to parameterized linear systems of the form $A(\mu) x(\mu) = b$ for many values of the parameter $\mu$. Here $A(\mu)$ is large, sparse, and nonsingular, with a nonlinear analytic dependence on $\mu$. Our approach is based on a companion linearization for parameterized linear systems. The companion matrix is similar to the operator in the infinite Arnoldi method, and we use this to adapt the flexible GMRES setting. In this way, our method returns a function $\tilde{x}(\mu)$ which is cheap to evaluate for different $\mu$, and the preconditioner is applied only approximately. This novel approach leads to increased freedom to carry out the action of the operation inexactly, which provides performance improvement over the method infinite GMRES, without a loss of accuracy in general. We show that the error of our method is estimated based on the magnitude of the parameter $\mu$, the inexactness of the preconditioning, and the spectrum of the linear companion matrix. Numerical examples from a finite element discretization of a Helmholtz equation with a parameterized material coefficient illustrate the competitiveness of our approach. The simulations are reproducible and publicly available online.

==> working_paper_precond_SC_EJ.tex <==
\maketitle
\begin{abstract}
\textbf{Need to write.} We consider linear parameter-dependent systems $A(\mu) x(\mu) = b$ for many different $\mu$, where $A(\mu)$ analytic, large and sparse with a nonlinear dependence on $\mu$.
\end{abstract}

\begin{keywords}
flexible preconditioning, parameter-dependent linear systems, Krylov methods, companion linearization, shifted linear systems, infinite Arnoldi
\end{keywords}

\section{Introduction}
%Problem formulation
\textbf{Must change order and stress novelty of method more.} We seek a the numerical solution to the large complex linear system
\begin{align} \label{eq:our-prob}
	A(\mu) x(\mu) = b,
\end{align}
where $A(\mu) \in \mathbb{C}^{n \times n}$ is analytic, $A(0)$ nonsingular and $b \in \mathbb{C}^n$ for $\mu \in \mathbb{C}$. The matrix $A(\mu)$ can be expressed in terms of a Taylor series expansion centered around origin with infinite terms, i.e.,
\begin{align} \label{eq:A-taylor}
	A(\mu) = \sum_{i=0}^{\infty} A^{(i)}(0) \frac{\mu^i}{i!}.
\end{align}
%Why we are interested in this solution
Solving large linear systems of equations of this form efficiently is a topic of great importance in most scientific fields involving computation. Large linear systems often arise from the application of the finite element method (FEM) to a partial differential equation (PDE), resulting in a large sparse system matrix. A finer FEM-discretization leads to higher accuracy and better modelling possibilities but also to larger systems. Thus, improving efficiency, accuracy and robustness of the method is critical \cite{Estep1996ComputationalDE}.

%In particular, we will look at
We are interested in obtaining the solution to \eqref{eq:our-prob} for many different $\mu$ simultaneously. In particular, we consider problems where the matrix $A(\mu)$ depends nonlinearly on the parameter $\mu$. Such problems arise naturally in the study of PDEs with uncertainty. \textbf{(Describe PDEs you look at.)}

%Our method is based on GMRES (citations) and summarized as follows
The new method presented here is based on the well-established GMRES method for linear systems \cite{Saad:1986:GMRES}. The main idea of our approach is summarized as follows. In order to handle the nonlinearity in \eqref{eq:our-prob} we use a technique called companion linearization which is very commonly used to analyze polynomial eigenvalue problems (PEPs). As a consequence of Theorem~\ref{theorem:linearization}, the solution to \eqref{eq:our-prob} and the parameterized system with linear dependence on $\mu$
\begin{align} \label{eq:K-M-c}
	(K-\mu M)v(\mu) = c
\end{align}
are equivalent in a certain sense. More specifically, \eqref{eq:K-M-c} is given by
\begin{align} \label{eq:lin}
	\left(
	\underbrace{\begin{bmatrix}
	A_0 & A_1 & A_2 & \cdots \\
	& I & & \\
	& & I & \\
	& & & \ddots
	\end{bmatrix}}_{K}
	- \mu
	\underbrace{\begin{bmatrix}
	0 & 0&\cdots & 0 \\
	I & & & \\
	& I & & \\
	& & \ddots & 0
	\end{bmatrix}}_{M}
	\right)
	\underbrace{\begin{bmatrix}
	x(\mu) \\
	\mu x(\mu) \\
	\mu^2 x(\mu) \\
	\vdots \\
	\end{bmatrix}}_{v(\mu)}
	=
	\underbrace{\begin{bmatrix}
	b \\
	0 \\
	0 \\
	\vdots
	\end{bmatrix}}_{c},
\end{align}
where $K, M$ constant matrices of infinite dimension, $c$ constant vector of infinite dimension. The matrix $K$ contains the Taylor series expansion coefficient matrices for $A(\mu)$ as in \eqref{eq:A-taylor}, i.e.,
\begin{align} \label{eq:Ai}
	A_i = \frac{1}{i!} A^{(i)}(0) \in \mathbb{C}^{n \times n}, \text{ } i=0,1,\ldots.
\end{align}
%Inexact preconditioning with dynamic stopping criteria (citations) and why
For $K$ nonsingular, right preconditioning matrix $K^{-1}$ transforms \eqref{eq:lin} as follows.
\begin{subequations}
\begin{eqnarray} \label{eq:transformation}
	&&(K-\mu M)v(\mu) = c \label{eq:unshifted} \\
	\iff \quad &&(K-\mu M)K^{-1}K v(\mu) = c \\
	\iff \quad &&(I - \mu M K^{-1}) \hat{v}(\mu) = c,  \label{eq:shifted}
\end{eqnarray}
\end{subequations}
with $\hat{v} = K v(\mu)$. In this paper we will consider solving equation \eqref{eq:shifted} by applying $K^{-1}$ inexactly via an iterative method, on each iteration of the Arnoldi method, i.e., in a flexible setting as developed in \cite{Saad1993}. In this way, we can vary how accurately we apply the preconditioner, leading to a large decrease in complexity compared to applying a preconditioner exactly on each iteration of the Arnoldi method.

To what tolerance level we apply the preconditioner is determined by a dynamic inner stopping criteria. In general, the preconditioner will be applied almost exactly when the dimension of the Krylov subspace is small, and with decreasing accuracy as the dimension of the subspace grows. The theory for this has been investigated and developed in \cite{Golub1999InexactPC,Simoncini2002a,inexKry}. This strategy differs from other inexact methods, where the inner tolerance has to stay at least constant \cite{FS1992}, or needs to decrease as the iterates become closer to the solution \cite{DET1982,Sherman1978}.

%We use shifted Krylov subspaces (citations) and why we are doing this
Krylov subspaces are invariant under shifts, a property previously shown to be useful in other works on parameterized linear systems \cite{Bahkos:2017:MULTIPREC,Baumann2015NestedKM, GuSimoncini, KressnerToblerLR, etna_vol45_pp499-523,SOODHALTER2014105}. Our linearization allows us to consider just one Krylov subspace formed independently of $\mu$ by a linear combination of the power sequence associated with the matrix $MK^{-1}$ and the vector $c$, i.e.,
\begin{align} \label{eq:our-krylov}
	\mathcal{K}_j (MK^{-1},b) := \{ c, MK^{-1}, \ldots, (MK^{-1})^{j-1}c \}.
\end{align}
We reuse the associated basis matrix to compute the $v(\mu)$ for all values of $\mu$. This amounts to additionally solving one least squares problem for every value of $\mu$ we consider.

%We used Infinite Arnoldi (citations) and why we are doing this
The Krylov subspace in \eqref{eq:our-krylov} has a particular structure which has been heavily exploited for NEP-methods, e.g. the infinite Arnoldi method \cite{Jarlebring:2012:INFARNOLDI} and various improvements thereof \cite{doi:10.1002/nla.2043,Jarlebring:2014:SCHUR,DelayProblem,TensorArnoldi,Mele2018}. We will show that this structure allows us to express $A(\mu)$ without truncation error in the Taylor series expansion, while carrying out the algorithm with a finite number of linear algebra operations.

%We used Infinite Arnoldi (citation), could have considered other NEP methods (citations)
Although we have focused on the flavors of the NEP-method
infinite Arnoldi method, there are many algorithms for NEPs that may also lead to competitive approaches, e.g., CORK \cite{VanBeeumen:2015:CORK} or TOAR \cite{Kressner:2014:TOAR}.

%Organization of the paper
This paper is organized as follows. \textbf{Need to write this.}

\section{Preliminaries}
\subsection{Truncated problem and notation}
%Define some notation used later
In this work, we will first consider a truncated problem before solving for the numerical solution to equation \eqref{eq:our-prob}. We define the truncated truncated parameterized system as
\begin{align} \label{eq:our-prob-trunc}
	A_m (\mu) x_m (\mu) = b,
\end{align}
where
\begin{align} \label{eq:A-trunc}
	A_m(\mu) = \sum_{i=0}^m A^{(i)} (0) \frac{\mu^i}{i!}
\end{align}
and truncated matrices $K_m$ and $M_m$ as
\begin{align} \label{eq:Km}
	K_m :=
	\begin{bmatrix}
		A_0 & A_1 & A_2 & \cdots & A_m \\
		& I & & & \\
		& & I & & \\
		& & & \ddots & \\
		& & & & I
	\end{bmatrix} \in \CC^{(m+1)n \times (m+1)n}
\end{align}
and
\begin{align} \label{eq:Mm}
	M_m :=
	\begin{bmatrix}
		0 & 0 & \cdots & 0 & 0\\
		I & & & & \\
		& I & & & \\
		& & \ddots & & 0 \\
		& & & I &
	\end{bmatrix} \in \CC^{(m+1)n \times (m+1)n},
\end{align}
where $K_m$ contains the first $(m+1)$ coefficients in the Taylor series expansion of $A(\mu)$. The truncated version the right-hand side vector $c$ as in \eqref{eq:lin} is defined as
\begin{align} \label{eq:cm}
	c_m := \begin{bmatrix} b, 0, \ldots, 0 \end{bmatrix}^T \in \CC^{(m+1)n}
\end{align}
and the truncated version of the matrix $K^{-1}$ is a block triangular matrix, which exists if $A_0$ nonsingular. This matrix is expressed exactly as
\begin{align} \label{eq:Km-inv}
	K_m^{-1} =
	\begin{bmatrix}
	A_0^{-1} & -A_0^{-1} A_1 & \cdots & -A_0^{-1} A_m  \\
	& I & & \\
	& & \ddots & \\
	& & & I
	\end{bmatrix} \in \CC^{(m+1)n \times (m+1)n}.
\end{align}
%The truncated matrix product $M_m K_m^{-1}$ is given by
%\begin{align} \label{eq:MK-inv}
%	M_m K_m^{-1} =
%	\begin{bmatrix}
%	0 & 0 & 0 & \cdots & 0 \\
%	A_{0}^{-1}& -A_{0}^{-1}A_1 & -A_{0}^{-1} A_2 & \cdots & -A_{0}^{-1}A_m \\
%	& I & & & \\
%	& & \ddots & & \\
%	& & & I & 0
%	\end{bmatrix} \in \CC^{(m+1)n \times (m+1)n}.
%\end{align}
We express the truncated version of equation \eqref{eq:unshifted} as
\begin{align} \label{eq:unshifted-trunc}
	\left(  K_m - \mu M_m \right) v_m (\mu) = c_m
\end{align}
and the truncated version of equation \eqref{eq:shifted} by
\begin{align} \label{eq:shifted-trunc}
	\left( I - \mu M_m K_m^{-1} \right) \hat{v}_m(\mu) = c_m,
\end{align}
where $K_m$ as in \eqref{eq:Km}, $M_m$ as in \eqref{eq:Mm}, $M_m K_m^{-1}$ as in \eqref{eq:MK-inv}, $\hat{v}_m = K_m v_m(\mu)$ and $c_m$ as in \eqref{eq:cm}. The vectorization operation is defined as the stacking of the columns into a vector, i.e. for any $W = \begin{bmatrix} w_0, w_1, \ldots, w_m \end{bmatrix} \in \CC^{n \times (m+1)}$,
\begin{align} \label{eq:vectorize}
	\vectorize(W) := \begin{bmatrix} w_0^T, w_1^T, \ldots, w_m^T \end{bmatrix}^T
\end{align}
and the matrix $\tilde{D}_m$ is defined as
\begin{align} \label{eq:tilde-D-m}
	\tilde{D}_m :=
	\begin{bmatrix}
	0 & 1 &  & & \\
	   &    & \ddots & & \\
	   & & &1 & 0
	\end{bmatrix} \RR^{(m-1) \times (m+1)}
\end{align}
where $\tilde{D}_1 := 0 \in \RR$. We denote the $m$-th largest singular value of a matrix $A \in \CC^{n_1 \times n_2}$ as $\sigma_m(A)$ and
\begin{align} \label{eq:polynom}
	\mathcal{P}_j^0 := \{ \text{polynomials } p \text{ of degree} \leq j \text{ with } p(0) = 1 \}.
\end{align}

\subsection{Companion linearization}
%Carefully explain the linearization and prove that the solution to our problem is equivalent to linearization
Companion linearizations has been extensively used for PEPs (see, e.g., \cite{Mackey:2006:VECT}) but also for linear systems \cite{GuSimoncini,JarlebringCorrenty1}. We now show how companion linearization can be applied leading to
a matrix structure that is also present in the infinite Arnoldi method, where it was be used to dynamically expand the linearization.

\begin{theorem} \label{theorem:linearization}
Suppose $A(\mu)$ as in \eqref{eq:our-prob} with truncated expansion as in \eqref{eq:A-trunc}. Then, the solutions to \eqref{eq:our-prob-trunc} and \eqref{eq:unshifted-trunc} are equivalent in the following sense.
\begin{enumerate}
\item[(a)] If solutions to \eqref{eq:unshifted-trunc} are of the form
\begin{align} \label{eq:our-vm}
	v_m(\mu) = \begin{bmatrix} \mu^0 x(\mu), \mu x(\mu), \ldots, \mu^m x(\mu) \end{bmatrix}^T
\end{align}
then $x_m(\mu)$ satisfies \eqref{eq:our-prob-trunc}
\item[(b)] If $x_m(\mu)$ satisfies \eqref{eq:our-prob-trunc} then $v_m(\mu)$ as in \eqref{eq:our-vm} satisfies \eqref{eq:unshifted-trunc}.
\end{enumerate}
\end{theorem}

\begin{proof}
\begin{enumerate}
\item[(a)] Assume \eqref{eq:unshifted-trunc} holds. Then, the first block row in \eqref{eq:unshifted-trunc} implies equation \eqref{eq:our-prob-trunc} is fulfilled.
\item[(b)] Assume \eqref{eq:our-prob-trunc} holds. Then, first block row in \eqref{eq:unshifted-trunc} satisfied. The $i$-th block row gives
\[
	\mu^{i-1} x_m(\mu) - (\mu) \mu^{i-2} x_m(\mu) = 0
\]
for $i=2,\ldots,m+1$.
\end{enumerate}
\end{proof}
Clearly, we can take $m \rightarrow \infty$ in Theorem~\ref{theorem:linearization}, obtaining that \eqref{eq:our-prob} and \eqref{eq:lin} are equivalent in an analogous sense.

\section{Algorithm}

\subsection{Flexible GMRES} \label{sec:FGMRES}
%A derivation of the flexible GMRES algorithm
As a preparation for the derivation of the proposed algorithm, we consider flexible preconditioning of the GMRES algorithm \cite{Saad1993}. For better efficiency of the linear system solver, Krylov subspace methods are commonly carried out on a preconditioned system where convergence is closer to optimal. This requires additional solutions to inner systems, which if selected well, results in a more efficient method. This is the foundation for the method flexible GMRES (FGMRES), which solves the resulting inner systems inexactly, thus resulting in faster convergence. FGMRES is summarized below. For a full explanation of the standard GMRES algorithm, see \cite{Saad:1986:GMRES}.

On the $j$-th iteration of the standard GMRES algorithm performed on the system $Ax = b$, with $A \in \CC^{n \times n}$, $b \in \CC^n$, we form the Arnoldi factorization
\[
	AQ_j = Q_{j+1} \underline{H}_j,
\]
where $Q_j = \begin{bmatrix} q_1,\ldots,q_j \end{bmatrix} \in \CC^{n \times j}$ is a matrix whose columns form an orthonormal basis for the Krylov subspace of dimension $j$ associated with the matrix $A$ and vector $b$ (see \eqref{eq:our-krylov}) and $\underline{H}_j \in \CC^{(j+1) \times j}$ upper Hessenberg. In practice, we perform one matrix vector product, $y = A q_j$ with $q_1 = b/ \norm{b}$, and orthogonalize this vector against the columns of $Q_j$ by a Gram-Schmidt process. This new vector is used to form $Q_{j+1}$. The orthogonalization coefficients are stored in $\underline{H}_j$. We compute the $j$-th iterate $x_j$ as
\[
	x_j = x_0 + Q_j w_j
\]
where
\begin{subequations}
\begin{eqnarray} \label{eq:comp-y}
	w_j &=& \argmin_{w} \norm{\beta e_1 - \underline{H}_j w}_2 \\
	\beta &=& \norm{b-Ax_0}_2
\end{eqnarray}
\end{subequations}
and $x_0$ is the initial iterate.
The basic idea behind preconditioned Krylov subspace methods is to solve a modified system of the form
\[
	A M^{-1} (Mx) = b,
\]
where $M \in \CC^{n \times n}$ nonsingular. In general, we do not need to form the matrix $AM^{-1}$ explicitly. The action of this matrix can instead be computed by solving the linear system
\begin{align} \label{eq:pre-con-step}
	Mz_i=q_i
\end{align}
for $i=1,\ldots,j$ and on iteration $j$ forming the Arnoldi factorization
\begin{align} \label{eq:pre-arn}
	A M^{-1} Q_j = Q_{j+1} \underline{H}_j.
\end{align}
The $j$-th iterate of preconditioned GMRES is thus given by
\[
	x_j = x_0 + M^{-1} Q_j w_j
\]
where $w_j$ is as in \eqref{eq:comp-y} and $\underline{H}_j$ as in \eqref{eq:pre-arn}. For efficiency, it is important that \eqref{eq:pre-con-step} is easy to compute for each vector $q_i$, for example by means of an iterative method.

The FGMRES method instead considers changing the preconditioner on each step of the Arnoldi algorithm, i.e., \eqref{eq:pre-con-step} is replaced by
\begin{align} \label{eq:pre-con-step2}
	M_i \tilde{z}_i=q_i
\end{align}
for $i=1,\ldots,j$ and on iteration $j$ we form the Arnoldi factorization
\begin{align} \label{eq:flex-arn}
	A \tilde{Z}_j = Q_{j+1} \underline{H}_j,
\end{align}
where $\tilde{Z}_j = \begin{bmatrix} \tilde{z}_1,\ldots, \tilde{z}_j \end{bmatrix}$. Here we take as before $q_1 = b/ \norm{b}$. The $j$-th iterate of FGMRES is thus given by
\[
	x_j = x_0 + \tilde{Z}_j w_j,
\]
where $w_j$ is computed as in \eqref{eq:comp-y} and $\underline{H}_j$ is as in \eqref{eq:flex-arn}.

In this paper, we consider the solution to the shifted system. Using the shift-invariance property of Krylov subspaces, i.e.,
\begin{align} \label{eq:shift-inv}
	\mathcal{K}_k (AM^{-1},b) = \mathcal{K}_k (I - \mu A M^{-1}, b),
\end{align}
leads to a shifted Arnoldi factorization of the form
\begin{align*}
	(I - \mu A M^{-1}) Q_j = Q_{j+1} (\underline{I}_j - \mu \underline{H}_j)
\end{align*}
in the general case and
\begin{align} \label{eq:shifted-arn}
	(I - \mu A) \tilde{Z}_j = Q_{j+1} (\underline{I}_j - \mu \underline{H}_j)
\end{align}
in the flexible form, where
\begin{align} \label{eq:Im}
	\underline{I}_j \in \RR^{(j+1) \times j}
\end{align}
is an identity matrix with an extra row of zeros. The $j$-th iterate of Flexible GMRES for the shifted system is thus given by $x_j$ where
\begin{subequations} \label{eq:der-least-squares}
\begin{eqnarray}
	w_j &=& \argmin_w \norm{\beta e_1 - (\underline{I}_j - \mu \underline{H}_j)w}_2 \\
	x_j &=& x_0 + \tilde{Z}_j w_j
\end{eqnarray}
\end{subequations}
and $\underline{H}_j$ is as in \eqref{eq:shifted-arn}. The FGMRES method thus requires the extra storage of the matrix $\tilde{Z}_j \in \CC^{n \times j}$ but no additional cost in computation compared to preconditioned GMRES.

%\subsection{An extension to infinity}
\subsection{Infinite flexible GMRES}
%Explain what makes it infinite since we will use this in the following subsection
\subsubsection{Algorithm derivation} \label{sec:Algder}
%Some text on:
% Apply standard FMGRES for shifted systems to (1.4) and exploit structure
We specialize the flexible GMRES algorithm described in Section~\ref{sec:FGMRES} for shifted systems to the system in equation \eqref{eq:unshifted-trunc} with an inexact application of the preconditioner $K_m^{-1}$. The structure of our linearization allows for an efficient computation of the corresponding Arnoldi factorization. Here we show the action of an operator of size $(m+1)n \times  (m+1)n$ can be achieved using vectors and matrices of size $n \times n$ and smaller. 

The standard preconditioned GMRES algorithm applied to \eqref{eq:unshifted-trunc} requires the Arnoldi factorization
\begin{align} \label{eq:shift-arn-our}
	\left( I - \mu M_m K_m^{-1} \right) Q_j = Q_{j+1} \left( \underline{I}_j - \mu \underline{H}_j \right),
\end{align}
formed by computing the product
\begin{align} \label{eq:multMK}
	M_m K_m^{-1} q_i
\end{align} where
on the $i$-th iteration of the Arnoldi method. This step is followed by an orthogonalization procedure and an update of the approximation via the computation of a least squares solution analogous to \eqref{eq:der-least-squares}. Here $q_1 = c_m/\norm{c_m}$ as in \eqref{eq:cm}, $Q_j \in \CC^{(m+1)n \times j}$ and $\underline{I}_j$ as in \eqref{eq:Im} and $\underline{H}_j \in \CC^{(j+1) \times j}$. The matrix $M_m K_m^{-1}$ is given by
\begin{align} \label{eq:MK-inv}
	M_m K_m^{-1} =
	\begin{bmatrix}
	0 & 0 & 0 & \cdots & 0 \\
	A_{0}^{-1}& -A_{0}^{-1}A_1 & -A_{0}^{-1} A_2 & \cdots & -A_{0}^{-1}A_m \\
	& I & & & \\
	& & \ddots & & \\
	& & & I & 0
	\end{bmatrix} \in \CC^{(m+1)n \times (m+1)n}. 
\end{align}
Consider first the action of the truncated matrix product $M_m K_m^{-1}$ where $K_m^{-1}$ is as in \eqref{eq:Km-inv}. From equation \eqref{eq:multMK} it is clear that in forming the Arnoldi factorization we must apply $A_0^{-1}$ to a new vector of size $n$ on each iteration. 

In a flexible GMRES setting, we apply an approximation of the preconditioning matrix on each iteration. For our specialization, this corresponds to approximating the action of $A_0^{-1}$ on each iteration, denoted $\tilde{A}_{0}^{-1}$, where the approximation is permitted to change from one iteration to the next. This modification does not change the structure of the matrix in \eqref{eq:MK-inv}. We denote the $i$-th preconditioning matrix as $\tilde{K}_{m_i}^{-1}$ and the shifted inexact Arnoldi factorization on iteration $j$ is given by
\begin{align} \label{eq:shift-in-trunc-arn}
	Q_j - \mu M_m \tilde{Z}_j = Q_{j+1} (\underline{I}_j - \mu \underline{H}_j),
\end{align}
where
\begin{align} \label{eq:flex-mult}
	\tilde{z}_i = \tilde{K}^{-1}_{m_i} q_i,
\end{align}
$\tilde{Z}_j = \begin{bmatrix} \tilde{z}_1, \ldots, \tilde{z}_j \end{bmatrix} \in \CC^{(m+1)n \times j}$ and $M_m$ as in \eqref{eq:Mm}.

%We consider the structure of the matrices $Q_m$ and $\tilde{Z}_m$.
The following theorem characterizes the important structure of the matrices $Q_i$ and $\tilde{Z}_i$, which will be proven as a consequence of the more technical result Lemma~\ref{matvec}.
\begin{theorem} \label{lemma1}
If we apply Flexible GMRES to the system in equation \eqref{eq:shifted-trunc} with an approximation (or an exact application) of $A_0^{-1}$ on each iteration, the nonzero structure in both $Q_i$ and $\tilde{Z}_i$ as in \eqref{eq:shift-in-trunc-arn}  (or $K_m^{-1} Q_i$ as in \eqref{eq:shift-arn-our}) grows by one block in each iteration $i=1,\ldots,j$.
\end{theorem}

We show in the following Lemma that the action of an operator of $M_m \tilde{K}_m^{-1}$ (or $M_m K_m^{-1}$) can be computed efficiently. Proofs of Lemma~\ref{matvec} and Theorem~\ref{lemma1} (respectively) follow after.
\begin{lemma} \label{matvec}
Let $M_m \tilde{K}_m^{-1}$ be as in \eqref{eq:MK-inv} with approximation $\tilde{A}_0^{-1}$. For any $W = \begin{bmatrix} w_0, w_1, \ldots, w_m \end{bmatrix} \in \CC^{n \times (m+1)}$
\[
    M_m \tilde{K}_m^{-1} \vectorize(W) = \vectorize(\bar{0}, \tilde{w}, W \tilde{D}_m^T) \in \CC^{n(m+1)},
\]
where
\begin{equation} \label{eq:tilde-w-small}
    \tilde{w} = \tilde{A}_0^{-1} w_0 -\tilde{A}_0^{-1} \left(\sum_{i=1}^{m} A_i w_i \right) \in \CC^{n},
\end{equation}
$\bar{0} \in \RR^{n}$ and $\tilde{D}_m$ as in \eqref{eq:tilde-D-m}.
\end{lemma}
%\begin{align} \label{eq:tilde-w-small}
%	\tilde{w} = \tilde{A}_0^{-1} w_0 -\tilde{A}_0^{-1} \left( \sum_{i=1}^k A_i w_i \right) \in \CC^n.
%\end{align}
\begin{proof}
Lemma~\ref{matvec} is proved as follows. We rewrite the product between the matrix in \eqref{eq:MK-inv} with approximation $\tilde{A}_0^{-1}$ and $\vectorize(W)$ as
\[
	M_m \tilde{K}_m^{-1} \vectorize(W) =
	\begin{bmatrix}
	\left(e^T \otimes D_0 \right) \vectorize(W)  \\
	\left(\tilde{A}_0^{-1} \left[ I, -A_1, -A_2, \ldots, -A_m \right]\right) \vectorize(W) \\
	\left(\tilde{D}_m \otimes I\right)\vectorize(W)
	\end{bmatrix},
\]
where $e=\begin{bmatrix}1,\ldots,1\end{bmatrix}^T \in \RR^{m+1}$ and
\begin{align*}
	D_0 =
	\begin{bmatrix}
	0 & \cdots & 0 \\
	\vdots & \ddots & \vdots \\
	0 & \cdots & 0
	\end{bmatrix} \in \RR^{n \times n}
\end{align*}
and $\tilde{D}_m$ is as in \eqref{eq:tilde-D-m}. The first block row can be expressed as
\[
	\vectorize(D_0 W e) = \begin{bmatrix} 0, \ldots, 0\end{bmatrix}^T \in \RR^{n},
\]
where we have used that $(X^T \otimes Y) \vectorize(Z)= \vectorize(YZX)$. Computing the second block row amounts to the following.
\[
	\tilde{A}_0^{-1} \left( w_0 -A_1 w_1 -A_2 w_2 -\ldots -A_m w_m \right) = \tilde{A}_0^{-1} w_0 - \tilde{A}_0^{-1} \sum_{i=1}^m A_i w_i \in \RR^{n}
\]
The remaining product is computed as
\[
	\left(\tilde{D}_m \otimes I\right)\vectorize(W) = \vectorize(W \tilde{D}_m^T) = \vectorize( \begin{bmatrix} w_1,\ldots,w_{m-1} \end{bmatrix}) \in \RR^{n(m-1)}.
\]

\begin{comment}
If $W$ as in \eqref{eq:small-W}, the second block row simplifies to
\begin{align*}
	\tilde{A}_0^{-1} \left( w_0 -A_1 w_1 -A_2 w_2 - \ldots- A_k w_k \right) = \tilde{A}_0^{-1} w_0 - \tilde{A}_0^{-1} \sum_{i=1}^k A_i w_i \in \RR^{n}
\end{align*}
and the remaining product can be written as
\[
	\left(\tilde{D}_m \otimes I\right)\vectorize(W) = \vectorize(\hat{W} \tilde{D}_k^T) = \vectorize( \begin{bmatrix} w_1,\ldots,w_{k-1}, 0, \ldots, 0 \end{bmatrix}) \in \RR^{n(m-1)}.
\]
\end{comment}

\end{proof}

Note that if $W$ is of the form
\begin{align} %\label{eq:small-W}
	W = \begin{bmatrix} \hat{W},0, \dots ,0 \end{bmatrix} \in \CC^{n \times (m+1)}, \text{ }
	\hat{W} = \begin{bmatrix} w_0, \ldots, w_k \end{bmatrix} \in \CC^{n \times (k+1)}
\end{align}
with $k < m$, then by a direct consequence of Lemma~\ref{matvec}, the matrix vector product reduces to
\begin{align} \label{eq:smaller-prod}
	M_m \tilde{K}_m^{-1} \vectorize{(W)} = \vectorize{(\bar{0}, \tilde{w}, \hat{W} \tilde{D}_{k}^T,0, \dots ,0)} \in \CC^{n(m+1)},
\end{align}
where $\tilde{w}$ is given by \eqref{eq:tilde-w-small} with $m$ replaced by $k$. 

\begin{proof}
Theorem~\ref{lemma1} is proved by the following reasoning. Take $q_1=c_m/\norm{c_m}$ with $c_m$ as in \eqref{eq:cm}. A direct result of Lemma~\ref{matvec} is the structure of the resulting vector is changed only by an expanding the number of nonzero entries in the first block, and the tail of zeros is preserved after orthogonalization (structure of $Q_i$). The same result holds for $\tilde{Z}_i$, where we require the matrix vector product in \eqref{eq:flex-mult} on each iteration. The matrix here has a block diagonal structure and thus the nonzero structure is preserved after multiplication.
\end{proof}

To visualize Theorem~\ref{lemma1} and Lemma~\ref{matvec}, consider the matrix vector products in the Arnoldi factorization in \eqref{eq:shift-in-trunc-arn} started on the vector $c_m$ as in \eqref{eq:cm}. The first product is given by
\begin{align*} %\label{eq:first-product}
	\begin{bmatrix}
	0 & 0 & 0 & \cdots & 0 \\
	\tilde{A}_{0}^{-1}& -\tilde{A}_{0}^{-1}A_1 & -\tilde{A}_{0}^{-1} A_2 & \cdots & -\tilde{A}_{0}^{-1}A_m \\
	& I & & & \\
	& & \ddots & & \\
	& & & I & 0
	\end{bmatrix}
	\begin{bmatrix}
	b \\
	0 \\
	0 \\
	\vdots \\
	0
	\end{bmatrix} =
	\begin{bmatrix}
	\bar{0} \\
	\tilde{A}_0^{-1} b \\
	0 \\
	\vdots \\
	0
	\end{bmatrix},
\end{align*}
and subsequent multiplications by
\begin{align} \label{eq:star}
	\begin{bmatrix}
	0 & 0 & 0 & \cdots & 0 \\
	\tilde{A}_{0}^{-1}& -\tilde{A}_{0}^{-1}A_1 & -\tilde{A}_{0}^{-1} A_2 & \cdots & \cdots & -\tilde{A}_{0}^{-1}A_m \\
	& I & & & & & \\
	& & \ddots & & & & \\
	& & & & & & \\
	& & & & \ddots & & \\
	& & & & &  I & 0
	\end{bmatrix}
	\begin{bmatrix}
	* \\
	\vdots \\
	* \\
	0 \\
	0 \\
	\vdots \\
	0
	\end{bmatrix} =
	\begin{bmatrix}
	\bar{0} \\
	* \\
	\vdots \\
	* \\
	0 \\
	\vdots \\
	0
	\end{bmatrix},
\end{align}
where the entries marked with $*$ represent nonzero blocks of dimension $n$. As the number of nonzero blocks grows by one on each iteration of the Arnoldi factorization, on the $j$-th iteration we have exactly $j$ nonzero blocks (i.e., $j$ $*$'s) in both vectors in equation \eqref{eq:star}. This structure is preserved after orthogonalization.

\begin{comment}
Elias comment:
** Elaborate on conversion of ``standard'' flexible GMRES to Algorithm~XX. Refer to formulas. **
** Refer to steps in Algorithm~XX: Repeated GS **
\end{comment}

The above process is summarized in Algorithm~\ref{alg:FIGMRES}, where we return a parametrized solution $\tilde{x}_j(\mu)$ as an approximation to equation \eqref{eq:our-prob}. We can evaluate this solution for many values of $\mu$ without running the algorithm again. Here we take $\tilde{x}_0(\mu) = 0 \in \RR^{n}$ and $q_1 = b/\norm{b} \in \CC^n$. Note that in Algorithm~\ref{alg:FIGMRES}, $q_i$ denotes only the nonzero elements above the tail of zeros. The nonzero elements of $\tilde{z}_i$, considering an inexact application of the preconditioner as in \eqref{eq:flex-mult}, can be expressed as
 \begin{align} \label{eq:z-tilde-for-alg}
 	\vectorize{(\tilde{w}, \hat{W} \tilde{D}_i)} \in \CC^{in}
 \end{align}
where $\vectorize{(\hat{W})} = \begin{bmatrix} q_i^T, \bar{0}^T \end{bmatrix}^T \in \CC^{(i+1)n}$, $q_i \in \CC^{in}$, $\bar{0} \in \CC^n$, $\tilde{w}$ as in \eqref{eq:tilde-w-small}, $\tilde{D}_i$ as in \eqref{eq:tilde-D-m}. The elements of $y = M \tilde{z}_i$ above the tail of zeros are given by
 \begin{align} \label{eq:y-for-alg}
 	\begin{bmatrix} \bar{0}^T, \tilde{z}_i^T \end{bmatrix}^T \in \CC^{(i+1)n}
 \end{align}
and the orthogonalization on line \ref{alg:gs-line1} is performed with a (possibly repeated) Gram-Schmidt procedure. Changing the last line of Algorithm~\ref{alg:FIGMRES} to
\begin{align} \label{eq:change_to_v}
    \tilde{v}_j (\mu): \mu \mapsto \tilde{Z}_j \argmin_{w \in \CC^j} \norm{ \left( \underline{I}_j - \mu \underline{H}_j \right) w - e_1 \norm{c} }_2
\end{align}
where $\tilde{v}_j(\mu) \in \CC^{(j+1)n}$ results in an approximation to the truncated system in equation \eqref{eq:unshifted-trunc}. Here we note that, in contrast to the standard flexible GMRES algorithm, we need only to store the first $n(i+1)$ elements in the resulting matrix-vector products instead of the full vectors.

\begin{algorithm}[h!]
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\SetKwFor{FOR}{for}{do}{end}
\Input{$m \in \mathbb{Z}^{+}$ the desired dimension of the Krylov subspace, \\ $A_i$, $i = 0,1,\ldots,j$ as in \eqref{eq:Ai}, \\ $b \in \CC^n$, \\ $\mu \in \CC \backslash \{ 0 \}$}
\Output{Approximate solution $\tilde{x}_j(\mu)$ to \eqref{eq:our-prob}}
$\tilde{Z}_0$ = empty matrix \\
$Q_1 = b/ \norm{b}$ \\
\FOR{$i = 1,2, \dots, j$}{
Compute nonzero elements of $\tilde{z}_i$ as in \eqref{eq:z-tilde-for-alg} \label{alg:Kinv} \\
Compute elements of $y$ above tail of zeros as in \eqref{eq:y-for-alg} \\
Orthogonalize $y$ against $q_1,\ldots,q_i$ by a Gram-Schmidt process \label{alg:gs-line1}  \\
    \nonl \Indp $h_i = Q_i^{T}y$ \\
    \nonl $y_{\perp} = y - Q_i h_i$ \\
    \Indm
    	Possibly repeat Step~\ref{alg:gs-line1} \\
    	Compute $\beta_i = ||y_{\perp}||$ \\
	Let $q_{i+1} = y_{\perp}/\beta_i$ \\
	Expand $Q_i$ by $n$ rows of zeros \\
	 $Q_{i+1} = [Q_i, q_{i+1}]$ \\
	Expand $\tilde{Z}_i = [\tilde{Z}_{i-1}, \tilde{z}_i]$ \\
	Let
	$\underline{H}_i =
    	\begin{bmatrix}
    	\underline{H}_{i-1} & h_i \\
    	0 & \beta_i
    	\end{bmatrix} \in \CC^{(i+1) \times i}$
}
Return function handle
\begin{align*}
    \tilde{x}_j (\mu): \mu \mapsto \tilde{Z}_j (1:n,:)  \argmin_{w \in \CC^j} \norm{ \left( \underline{I}_j - \mu \underline{H}_j \right) w - e_1 \norm{c} }_2
\end{align*}
\caption{Flexible Infinite GMRES}
\label{alg:FIGMRES}
\end{algorithm}

\subsubsection{Extension to infinity} \label{sec:ext-to-infty}

Note that Algorithm~\ref{alg:FIGMRES} is independent of the truncation parameter $m$. This is due to Lemma~\ref{matvec}. The number of operations to calculate the product in \eqref{eq:smaller-prod} is independent of the number of the length of the vector, assuming the structure consisting of a fixed number of nonzero blocks. Hence, in theory we can take $m \rightarrow \infty$ and compute the product of a vector with an infinite tail of zeros with an infinite companion matrix in a finite number of linear algebra operations. As in the proof of Theorem~\ref{lemma1}, the infinite tail of zeros on each of the resulting vectors are preserved even after orthogonalization. Hence, Algorithm~\ref{alg:FIGMRES} is equivalent to the application of standard flexible GMRES for parameterized linear systems applied to the infinite matrices corresponding to $m \rightarrow \infty$. This procedure is completely analogous as the infinite Arnoldi method \cite{Jarlebring:2012:INFARNOLDI}.

%As noted in Section~\ref{sec:Algder}, we store only the elements in the nonzero blocks. So, taking $m \to \infty$ does not require a change in Algorithm~\ref{alg:FIGMRES}.
Therefore, this process represents the Taylor series of $A(\mu)$ as in \eqref{eq:our-prob} without any truncation error, i.e., Algorithm~\ref{alg:FIGMRES} as written indeed approximates the solution in \eqref{eq:lin}. As a result, Algorithm~\ref{alg:FIGMRES} approximates equation \eqref{eq:our-prob} and not the truncated problem in equation \eqref{eq:our-prob-trunc}.

\begin{comment}
\subsection{Application of the flexible preconditioner}
%Explain what you do when you apply K^{-1} iteratively
Consider approximating the solution to \eqref{eq:our-prob} by solving the shifted preconditioned system \eqref{eq:shifted} with GMRES. Here we use the shift-invariance of Krylov subspaces and form the Arnoldi factorization
\begin{align} \label{eq:our-ex-arn}
	MK^{-1} Q_m = Q_{m+1} \underline{H}_m
\end{align}
expressed equivalently as
\[
	(I - \mu M K^{-1}) Q_m = Q_{m+1} (\underline{I}_m - \mu \underline{H}_m),
\]
as described in Section~\ref{sec:FGMRES}. Here $M$, $K^{-1}$ are infinite matrices and $Q_m$ is an orthogonal matrix with an infinite number of rows and $m$ columns. In order to compute \eqref{eq:our-ex-arn}, we must calculate the matrix vector products $MK^{-1} q_j$ for $j=1,\ldots,m$.

The preconditioning matrix $K^{-1}$ is block upper triangular matrix, expressed exactly as
\begin{align} \label{eq:Kinv}
	K^{-1} =
	\begin{bmatrix}
	A_0^{-1} & -A_0^{-1} A_1 & -A_0^{-1} A_2 & \cdots & \cdots \\
	& I & & \\
	& & I & \\
	& & & \ddots
	\end{bmatrix}.
\end{align}
Applying this preconditioner exactly on every Arnoldi iteration corresponds to computing
\begin{align}
	z_j = K^{-1} q_j  \label{eq:apply-pre-ex}.
\end{align}
We can express \eqref{eq:apply-pre-ex} using the notation of Theorem~\ref{matvec} as follows. For $j=1$,
\begin{align} \label{eq:apply-inv1}
	z_1 &= K^{-1} q_1 =
	\begin{bmatrix}
	-A_0^{-1} \left(-\hat{q}_{1_0} \right) \\
	0 \\
	0 \\
	\vdots
	\end{bmatrix}
\end{align}
where
\begin{align*}
	\tilde{q}_1 &=\begin{bmatrix} q_1, 0, \ldots \end{bmatrix} = \begin{bmatrix} \frac{b}{\norm{b}}, 0, \ldots \end{bmatrix} = \begin{bmatrix} \hat{q}_{1_0}, 0, \ldots \end{bmatrix}
\end{align*}
and the vector $b$ is as in \eqref{eq:lin}. The matrix $\tilde{q}_1$ has $n$ rows and an infinite number of columns and the vector $z_1$ is an infinite vector. Subsequently, for $j>1$,
\begin{align} \label{eq:apply-inv2}
	z_j &= K^{-1} q_j =
	\begin{bmatrix}
	-A_0^{-1} \left(-\hat{q}_{j_0} + \sum_{i=1}^{j-1} \hat{q}_{j_{i}} \right) \\
	\hat{q}_{j_1} \\
	\vdots \\
	\hat{q}_{j_{j-1}} \\
	0 \\
	0 \\
	\vdots
	\end{bmatrix}
\end{align}
with
\begin{align*}
	\tilde{q}_j &= \big[ \overbrace{q_{j_1}, \ldots, q_{j_n}}^{\hat{q}_{j_0}}, \overbrace{q_{j_{(n+1)}} \ldots, q_{j_{2n}}}^{\hat{q}_{j_1}}, \ldots, \overbrace{q_{j_{((j-1)n+1)}}, \ldots,q_{j_{(jn)}}}^{\hat{q}_{j_{j-1}}} , 0, \ldots \big] \\ &=\begin{bmatrix} \hat{q}_{j_0}, \hat{q}_{j_1}, \ldots, \hat{q}_{j_{j-1}}, 0, \ldots \end{bmatrix}.
\end{align*}
We note that, as in the case with $j=1$, the matrix $\tilde{q}_j$ has $n$ rows and an infinite number of columns, and $z_j$ is an infinite vector.

The first block rows in equations \eqref{eq:apply-inv1} and \eqref{eq:apply-inv2} show that we require the application of the matrix $A_0^{-1} \in \CC^{n \times n}$ on a unique vector on the $j$-th Arnoldi iteration. In other words, we require a linear solve each time we apply the preconditioning matrix $K^{-1}$. One option to handle this is to compute an LU factorization of the matrix $A_0$ and reuse this factorization on each iteration. A cheaper alternative is to consider an iterative solver for the application of $A_0^{-1}$, and to vary the tolerance each time it is applied. This corresponds to forming the Arnoldi factorization
\begin{align} \label{eq:inexact-arn}
	Q_m - \mu M \tilde{Z}_m = Q_{m+1} (\underline{I}_m - \mu \underline{H}_m)
\end{align}
on iteration $m$, where $\tilde{Z}_m = \begin{bmatrix} \tilde{z}_1, \ldots, \tilde{z}_m \end{bmatrix}$ and
\begin{align} \label{eq:tilde-z}
	\tilde{z}_j = \tilde{K}^{-1}_j q_j.
\end{align}
We note that each vector $\tilde{z}_j$ is an infinite vector and $\tilde{K}_j$ refers to an inexact and varying application of the preconditioning matrix as described above. This process is summarized in Algorithm~\ref{alg:FIGMRES}.
\end{comment}

\subsection{Dynamic inner stopping criteria} \label{sec:inner-tol}
%Explain rigorously what this entails
In \cite{inexKry} the authors show that a flexible preconditioner can be applied to lower levels of accuracy as the residual of the method decreases, without destroying convergence. In this way, a method is constructed which dynamically increases the tolerance in the application of the preconditioner as the algorithm progresses. This framework allows for a more efficient algorithm without sacrificing accuracy. We adapt this criteria to the application of the flexible preconditioner in Algorithm~\ref{alg:FIGMRES}. 

More specifically, on the $j$-th iteration of Algorithm~\ref{alg:FIGMRES} we form the inexact Arnoldi factorization \eqref{eq:shift-in-trunc-arn}. This is achieved by computing $\tilde{z}_i$ for $i=1,\ldots,j$ as in \eqref{eq:flex-mult}, i.e., via an inexact application of $A_0^{-1}$. As we are considering a flexible GMRES setting in Algorithm~\ref{alg:FIGMRES}, the application of $A_0^{-1}$ by an iterative method can be performed to different tolerance levels on each iteration of the Arnoldi algorithm. The following analysis shows how the accuracy of the application of $A_0^{-1}$ can be chosen dynamically. In particular, we can relax the tolerance on the application of $A_0^{-1}$ as the residual of the method decreases. 

Let $\tilde{v}_j (\mu) \in \mathbb{C}^{(j+1) \times n}$ be as in \eqref{eq:change_to_v}, i.e., the $j$-th parametrized approximation returned from Algorithm~\ref{alg:FIGMRES} applied to the system in equation \eqref{eq:unshifted-trunc}.  Assume $m \to \infty$, i.e., the system in equation \eqref{eq:unshifted-trunc} contains an infinite Taylor series expansion without truncation (see Section~\ref{sec:ext-to-infty}). On iteration $j$ we compute
\begin{subequations} \label{eq:two-eq}
\begin{eqnarray}
	w_j &=& \argmin_{w \in \CC^j} \norm{(\underline{I}_j - \mu \underline{H}_j)w - e_1 \norm{c_m}}_2 \label{eq:wm} \\
	\tilde{v}_j(\mu) &=& \tilde{Z}_j w_j
\end{eqnarray}
\end{subequations}
with $\tilde{Z}_j, \underline{H}_j$ as in \eqref{eq:shift-in-trunc-arn}. Note that  $\tilde{v}_j(\mu) \in \CC^{(m+1)n}$. The inner residual on the $i$-th Arnoldi iteration, denoted $p_i$, represents how inexactly we apply the preconditioning matrix $K_m^{-1}$ in a flexible setting, i.e.,
\begin{align} \label{eq:pj1}
	p_i = K_m \tilde{z}_i - q_i,
\end{align}
and thus in matrix form, we have
\begin{align} \label{eq:res-mat}
	K_m \tilde{Z}_j = Q_j + P_j,
\end{align}
where $P_j = \begin{bmatrix} p_1, \ldots, p_j \end{bmatrix}$ after $j$ iterations.

Thus, using \eqref{eq:shift-in-trunc-arn} and \eqref{eq:res-mat}, we express $r_j$, the residual of the $j$-th approximate solution to \eqref{eq:unshifted-trunc} as follows.
\begin{subequations}\label{eq:r-rtilde}
\begin{eqnarray}
	r_j &=&  c_m - (K_m - \mu M_m) \tilde{v}_j (\mu) \\
	&=& c_m - (K_m - \mu M_m) \tilde{Z}_j w_j \label{eq:line2} \\
	&=& c_m - K_m \tilde{Z}_j w_j + \mu M_m \tilde{Z}_j w_j \\
	&=& c_m - K_m \tilde{Z}_j w_j - \big( Q_{j+1} (\underline{I}_j - \mu \underline{H}_j) - Q_j \big) w_j \\
	&=& c_m - (Q_j + P_j ) w_j - Q_{j+1} (\underline{I}_j - \mu \underline{H}_j) w_j + Q_j w_j \\
	&=& Q_{j+1} \big( e_1 \norm{c_m} - (\underline{I}_j - \mu \underline{H}_j) w_j \big) - P_j w_j \\
	&=& \tilde{r}_j - P_j w_j \label{eq:separate}
\end{eqnarray}
\end{subequations}
We refer to the vector $\tilde{r}_j$ above as the residual of the underlying method. This vector expresses the residual at the $j$-th iteration under the assumption that the preconditioning matrix $K_m^{-1}$ is applied exactly on each iteration. Thus, in equation \eqref{eq:separate} we have separated the error introduced from the inexact preconditioning from the residual of the GMRES applied to the shifted system \eqref{eq:shifted-trunc}.

 As in \cite{inexKry}, we define the quantity
\begin{align} \label{eq:distance}
	\delta_j := \norm{r_j - \tilde{r}_j} = \norm{P_j w_j},
\end{align}
i.e., the distance between the true residual and the residual of the underlying method. A small value in equation \eqref{eq:distance} can be interpreted as the flexible GMRES algorithm produces an approximation close to the approximation produced by the standard preconditioned GMRES algorithm.

The following Proposition quantifies how large the norm of the inner residual, i.e., norm of the vector in equation \eqref{eq:pj1}, can be in order to guarantee a small value for the quantity $\delta_j$.

\begin{proposition} \label{prop1}
Let $\varepsilon > 0$ and $w_j = \begin{bmatrix} \eta_1^{(j)}, \ldots, \eta_j^{(j)} \end{bmatrix}^T \in \mathbb{C}^j$ as in \eqref{eq:wm}. Let the residual of Algorithm~\ref{alg:FIGMRES} applied to \eqref{eq:unshifted-trunc} on iteration $j$ be given as in \eqref{eq:line2} and the computed residual
\[
	\tilde{r}_i = Q_{i+1} \big( e_1 \norm{c_m} - (\underline{I}_i - \mu \underline{H}_i) w_i \big)
\]
for $i=1,\ldots,j$. If at each iteration $i \leq j$ the inner residual $p_i$ as in \eqref{eq:pj1}
satisfies
\begin{align} \label{eq:stop-crit}
	\norm{p_i} \leq \frac{ \sigma_j(\underline{I}_j - \mu \underline{H}_j)}{j} \frac{1}{\norm{\tilde{r}_{i-1}}} \varepsilon \equiv \varepsilon_{\text{inner}}
 \end{align}
then $\delta_j \leq \varepsilon$, where $\delta_j$ as in \eqref{eq:distance}.
\end{proposition}

\begin{proof}
A direct application of \cite[Lemma~5.1 and Proposition 9.1]{inexKry} gives the desired result. 

\begin{comment}
\[
	\abs{(w_j)_i} = \abs{\eta_i^{(j)}} \leq \frac{1}{\sigma_j (\underline{I}_j - \mu \underline{H}_j)} \norm{\tilde{r}_{i-1}}
\]
for $i=1,\ldots,j$. Then,
\begin{subequations}
\begin{eqnarray*}
	\delta_j &:=& \norm{r_j - \tilde{r}_j} \\
	&=& \norm{P_j w_j} \\
	&=& \norm{\eta_1^{(j)} p_1 + \eta_2^{(j)} p_2 + \ldots + \eta_j^{(j)} p_j} \\
	&\leq& \sum_{i=1}^j \abs{\eta_i^{(j)}} \norm{p_i} \\
	&\leq& \sum_{i=1}^j \left( \abs{\frac{1}{\sigma_j(\underline{I}_j - \mu \underline{H}_j)}} \norm{\tilde{r}_{i-1}} \norm{p_i} \right)  \\
	&=& \left( \frac{1}{\sigma_j(\underline{I}_j - \mu \underline{H}_j)} \right) \sum_{i=1}^j \left( \norm{\tilde{r}_{i-1}} \norm{p_i} \right) \\
	&\leq& \left( \frac{1}{\sigma_j(\underline{I}_j - \mu \underline{H}_j)} \right) \sum_{i=1}^j \left( \norm{\tilde{r}_{i-1}} \frac{\sigma_j(\underline{I}_j - \mu \underline{H}_j)}{j} \frac{1}{\norm{\tilde{r}_{i-1}}}\varepsilon \right) \\
	&=& \varepsilon.
\end{eqnarray*}
\end{subequations}
\end{comment}

\end{proof}

We note that we can express \eqref{eq:stop-crit} as
\begin{align} \label{eq:pj-ineq}
	\norm{p_i} \leq \ell_j \frac{1}{\norm{\tilde{r}_{i-1}}} \varepsilon \equiv \varepsilon_{\text{inner}},
\end{align}
for $i=1,\ldots,j$, where $\ell_j$ is a constant independent of $i$. Equation \eqref{eq:pj-ineq} can be interpreted as follows, assuming a small fixed $\varepsilon > 0$. The quantities $\norm{p_i}$ and $\norm{\tilde{r}_{i-1}}$ are inversely related, since
\begin{align} \label{eq:inverse}
	\norm{p_i} \norm{\tilde{r}_{i-1}} \approx \ell_j \varepsilon.
\end{align}
As $\norm{\tilde{r}_{i-1}}$ represents the norm of the residual of the underlying method, we can additionally interpret \eqref{eq:pj-ineq} as the smaller the norm of the residual of the underlying method, the more inexactly we can apply preconditioner $K_m^{-1}$ as in \eqref{eq:flex-mult}. In practice, this corresponds to applying the matrix $A_0^{-1}$ by an iterative method with an increasing tolerance as the algorithm progresses.

\section{Convergence theory}
%As $\tilde{Z}_m$ is not a basis for a Krylov subspace, we can no longer apply the traditional convergence theory of the method GMRES directly to our algorithm.
Our main interest is to apply Algorithm~\ref{alg:FIGMRES} to approximate \eqref{eq:our-prob} for many different values of $\mu$. We therefore examine the relationship between the performance of the algorithm and the magnitude of the parameter $\mu$. Consider the norm of the residual where we apply Algorithm~\ref{alg:FIGMRES} to \eqref{eq:unshifted-trunc}, i.e., on the $j$-th iteration we compute
\begin{align} \label{eq:big-res}
	\norm{r_j} = \norm{c_m - (K_m-\mu M_m) \tilde{v}_j(\mu)}
\end{align}
with $K_m$, $M_m$ and $c_m$ as in \eqref{eq:Km}-\eqref{eq:cm} and $\tilde{v}_j(\mu)$ is the $j$-th iterate of Algorithm~\ref{alg:FIGMRES} as in \eqref{eq:change_to_v}. We can express $\norm{r_j}$ in terms of the residual of the underlying method and an error term as in \eqref{eq:r-rtilde}, i.e.,
\begin{subequations}
\begin{eqnarray*}
	\norm{r_j} &=& \norm{Q_{j+1} \big( e_1 \norm{c_m} - (\underline{I}_j - \mu \underline{H}_j) w_j \big) - P_j w_j} \\
	&=& \norm{\tilde{r}_j - P_j w_j},
\end{eqnarray*}
\end{subequations}
where the matrices $Q_j$, $H_j$ are as in \eqref{eq:shift-in-trunc-arn} and the matrix $P_j$ contains the inner residual vectors as in \eqref{eq:pj1}. Thus,
\begin{align} \label{eq:r-ineq}
	\norm{r_j} \leq \norm{\tilde{r}_j} + \norm{P_j w_j}.
\end{align}
Consider first $\norm{\tilde{r}_j}$, which can be interpreted as the norm of the residual as in \eqref{eq:big-res} under the assumption that the preconditioning matrix $K_m^{-1}$ is applied exactly on each iteration of Algorithm~\ref{alg:FIGMRES}. Denote the approximation under this condition
\begin{align} \label{eq:u-tilde-i}
	\tilde{u}_i(\mu), i=1,\ldots,j.
\end{align}
Here we have
\[
	\tilde{Z}_j = K_m^{-1} Q_j,
\]
i.e., $P_j$ is the zero matrix. We express $\norm{\tilde{r}_j}$ as
\begin{subequations} \label{eq:calc-r-tilde}
\begin{eqnarray}
	\norm{\tilde{r}_j} &=& \norm{c_m - (K_m - \mu M_m) \tilde{u}_j (\mu)} \label{eq:norm-r-tilde} \\
	&=& \norm{c_m - (K_m - \mu M_m) K_m^{-1} K_m \tilde{u}_j (\mu)} \\
	&=& \norm{c_m - (I-\mu M_m K_m^{-1}) \hat{\tilde{u}}_j (\mu)},
\end{eqnarray}
\end{subequations}
where $\hat{\tilde{u}}_j(\mu) = K_m \tilde{u}_j (\mu)$. The following theorem gives a bound for $\norm{\tilde{r}_j}$.

\begin{theorem} \label{eq:theorem-res}
Suppose Algorithm~\ref{alg:FIGMRES} is executed with an inexact solve satisfying the criteria \eqref{eq:stop-crit}. Then, the residual vector at iteration $j$ satisfies
\begin{align} \label{eq:r-eq}
\|r_j\|\le \min_{p \in \mathcal{P}_j^0} \norm{p (I - \mu M_m K_m^{-1}) c_m} + \varepsilon, 
\end{align}
where $\mathcal{P}_j^0$ as in \eqref{eq:polynom}.
\end{theorem}


%\begin{corollary}
%Let $r_j^{\mu_1}(\mu_2)$ denote the execution of
%Algorith~1 using a stopping criteria based on $\mu_1$ and evaluated for $\mu_2$.
%Suppose  $\|\tilde{r}_j(\mu_2)\|<\|\tilde{r}_j(\mu_1)\|$ for all $j$, then
%\[
% \|r_j^{\mu_1}(\mu_2) \| \le \varepsilon+\min_{p \in \mathcal{P}_j^0} \norm{p (I - \mu_2 M_m K_m^{-1}) c_m}.
%\]
%\end{corollary}
%\begin{proof}
%In this notation Theorem 4.1 gives
%a bound on  $\|r_j^{\mu_1}(\mu_1) \|$.
%Idea: Show that the conditions for Theorem 4.1 with $\mu=\mu_2$ are satisfied.
%
%Since by assumption \eqref{eq:stop-crit} is satsfied for $\mu_1$:
%\[
%\|p_i\|
%\]
%\end{proof}
%\begin{theorem}
%Suppose also $A(\mu)$ as in \eqref{eq:our-prob} and the matrices in equations \eqref{eq:unshifted-trunc} and \eqref{eq:shifted-trunc} nonsingular. Let $c_m \in \CC^{(m+1)n}$ and $(I - \mu M_m K_m^{-1}) =V \Lambda V^{-1}$ be a Jordan decomposition.  Let $\tilde{u}_j$ as in \eqref{eq:u-tilde-i}, $\norm{\tilde{r}_j}$ as in \eqref{eq:calc-r-tilde}. Then, the residual vector at iteration $j$ satisfies
%\begin{align} \label{eq:r-tilde-eq}
%	\norm{\tilde{r}_j}  = \min_{p \in \mathcal{P}_j^0} \norm{p (I - \mu M_m K_m^{-1}) c_m} \leq \min_{p \in \mathcal{P}_j^0} \norm{V} \norm{V^{-1}} \norm{p (\Lambda)} \norm{c_m},
%\end{align}
%where $\mathcal{P}_j^0$ as in \eqref{eq:polynom}.
%\end{theorem}

Theorem~\ref{eq:theorem-res} is proved from applying the standard convergence theory of GMRES \cite{Saad:1986:GMRES} combined with Proposition~\ref{prop1}, where we showed $\norm{P_j w_j} \leq \varepsilon$. 

To illustrate Theorem~\ref{eq:theorem-res}, we rewrite equation \eqref{eq:r-eq} as
\begin{subequations}
\begin{eqnarray} 
	\norm{r_j} &\leq& \min_{p \in \mathcal{P}_j^0} \norm{p (I - \mu M_m K_m^{-1})c_m} + \varepsilon \\
	&\leq& \norm{q (I - \mu M_m K_m^{-1})c_m} + \varepsilon \label{eq:r-tilde-2}
\end{eqnarray}
\end{subequations}
where the polynomial $q$ is defined as
\[
	q(z) := \frac{(1-z)^{j-k} \prod_{i=1}^k (1- z - \mu \gamma_i)}{\prod_{i=1}^k (1-\mu \gamma_i)},
\]
and $\gamma_{k+1}$ is the ($k+1$)-th largest eigenvalue of $M_m K_m^{-1}$ in modulus. Here $q$ is a normalized degree $j$ Zarantonello polynomial \cite{ZaranVarga}. The inequality in equation \eqref{eq:r-tilde-2} can thus be rewritten as
\begin{align} \label{eq:r-tilde-bound}
	\norm{r_j} \leq \norm{\frac{(\mu M_m K_m^{-1})^{j-k} \prod_{i=1}^k (\mu M_m K_m^{-1} - \mu \gamma_i)}{\prod_{i=1}^k (1-\mu \gamma_i)}} \norm{c_m} + \varepsilon,
\end{align}
and we obtain
\begin{align} \label{eq:conv-bound}
	\norm{r_j} \leq ( |\mu| |\gamma_{k+1}| )^j + \varepsilon
\end{align}
for sufficiently large $j$ (see \cite[Theorem~4.1]{JarlebringCorrenty1}). 

As noted in Section~\ref{sec:ext-to-infty}, as $m \rightarrow \infty$, Algorithm~\ref{alg:FIGMRES} as stated approximates the solution to equation \eqref{eq:lin} without truncation, i.e., approximates the solution to equation \eqref{eq:our-prob} without neglecting any of the terms in the infinite Taylor series expansion \eqref{eq:A-taylor}. Thus, error in the approximation comes then entirely from the iterative method. In practice, Algorithm~\ref{alg:FIGMRES} converges fast for small values of $\mu$.

\begin{comment}
Examining the second term on the right-hand side of \eqref{eq:r-ineq}, we express $w_j$ (see \eqref{eq:wm}) in terms of a solution to the normal equations, i.e.,
\[
	w_j = \left( (\underline{I}_j - \mu \underline{H}_j)^T (\underline{I}_j - \mu \underline{H}_j) \right)^{-1} (\underline{I}_j - \mu \underline{H}_j)^T e_1 \norm{c},
\]
expressed equivalently as
\begin{subequations}
\begin{eqnarray}
	w_j &=& \left( (\underline{I}_j^T - \mu \underline{H}_j^T) (\underline{I}_j - \mu \underline{H}_j) \right)^{-1} (\underline{I}_j^T - \mu \underline{H}_j^T) e_1 \norm{c} \\
	&=& \left( I - \mu \underline{I}_j^T \underline{H}_j - \mu \underline{H}_j^T \underline{I}_j + \mu^2 \underline{H}_j^T \underline{H}_j \right)^{-1} (\underline{I}_j^T - \mu \underline{H}_j^T) e_1 \norm{c} \\
	&=& \left( I + \mu \underline{I}_j^T \underline{H}_j + \mu \underline{H}_j^T \underline{I}_j - \mu^2 \underline{H}_j^T \underline{H}_j + \ldots \right) (\underline{I}_j^T - \mu \underline{H}_j^T) e_1 \norm{c}, \label{eq:taylor-ser}
\end{eqnarray}
\end{subequations}
where we have used the Taylor series expansion for $1/(1-x)$ for the equality on line \eqref{eq:taylor-ser}. Simplifying further gives
\begin{align} \label{eq:wj-equat}
	w_j = \left( (\underline{I}_j^T - \mu \underline{H}_j^T) + \mu \underline{I}_j^T \underline{H}_j (\underline{I}_j^T - \mu \underline{H}_j^T) + \mu \underline{H}_j^T \underline{I}_j (\underline{I}_j^T - \mu \underline{H}_j^T)  + \ldots \right) e_1 \norm{c},
\end{align}
and thus
\begin{align}
	w_j = e_1 \norm{c} + \mu \tilde{h}_j + \ldots \label{eq:lin-in-mu},
\end{align}
where the vector $\tilde{h}_j$ \color{red} (independent of $\mu$ since the Arnoldi factorization is done independently of $\mu$) \color{black} represents the product of the sum of the matrices where $\mu$ appears as a coefficient and the vector $e_1 \norm{c}$ in \eqref{eq:wj-equat}.

\color{red} Thus, for $\mu \rightarrow 0$, $w_j$ goes to $e_1 \norm{c}$ linearly in $\mu$ and, in the limit,
\begin{align} \label{eq:pj-wj-lim}
	\norm{P_j w_j} \leq \norm{P_j e_1 \norm{c}} = \norm{p_1 \norm{c}} \leq \varepsilon
\end{align}
\color{black} since the inequality in equation \eqref{eq:pj-ineq} for $j=1$ and $\ell_m=1$ gives
\[
	\norm{p_1} \leq \frac{1}{\norm{c}} \varepsilon
\]
and $\tilde{r}_0=c$. It is clear from equations \eqref{eq:r-ineq} and \eqref{eq:r-tilde-bound} along with the inequality in \eqref{eq:pj-wj-lim} that \color{red} for $\mu \rightarrow 0$
\begin{subequations}
\begin{eqnarray} \label{eq:conv-bound}
	\norm{r_j} &\leq \left( |\mu| \rho(MK^{-1}) \right)^j + \varepsilon \\
	&\leq \varepsilon
\end{eqnarray}
\end{subequations}
for sufficiently large $j$. \color{black}
\end{comment}

\begin{comment}
The vector $w_j$ is the solution to the linear least squares equation in \eqref{eq:wm}. Thus equation \eqref{eq:norm-r-tilde} can be interpreted as the norm of the residual of the exact same least squares problem. Considering the limit, i.e., $\mu \rightarrow 0$, we observe the following.
\begin{subequations} \label{eq:arrow-mu}
\begin{eqnarray}
	\argmin_{w \in \CC^j} \norm{(\underline{I}_j - \mu \underline{H}_j)w - e_1 \norm{c}}_2 &\xrightarrow[\mu \rightarrow 0]{}&
	 \argmin_{w \in \CC^j} \norm{\underline{I}_j w - e_1 \norm{c}}_2 \\ &=&  e_1 \norm{c}
\end{eqnarray}
\end{subequations}
In other words, the least squares problem becomes trivial as $\mu \rightarrow 0$. Thus,
\begin{align} \label{eq:lim-rtilde}
	\lim_{\mu \rightarrow 0} \norm{\tilde{r}_j} = 0.
\end{align}
The quantity in \eqref{eq:lim-rtilde} can be interpreted further as follows. Since \eqref{eq:arrow-mu} holds for all $j=1,\ldots,m$, the norm of the residual of the underlying method is small for small values of $\mu$, even when the dimension of the Krylov subspace is small.
\end{comment}
\begin{remark}[Different $\mu$ in evaluation and stopping criteria] \rm
Theorem 4.1 states the convergence of Algorithm~1 based on a stopping criteria
involving $\mu$ and evaluation of the approximation the linear system for that $\mu$. In practice we want to use the parameterization for many different other $\mu$, and need to use a specific $\mu$ in the stopping criteria. The above theory suggests that smaller $\mu$ implies that $\tilde{r}_j$ converges faster. This in turn implies that the bound \eqref{eq:pj-ineq} for a smaller $\mu$ becomes less strict, i.e., in general we expect that if we use $\mu$ for the stopping criteria, the algorithm will
also work for smaller $\mu$.
\end{remark}

\section{Simulations}
\subsection{Illustration of the theory}
We consider approximating the solution to \eqref{eq:our-prob} with Algorithm~\ref{alg:FIGMRES}, where
\begin{align} \label{eq:delay-A}
	A(\mu) = -\mu I + A_0 + A_1 e^{-\mu},
\end{align}
with $A_0, A_1 \in \RR^{n \times n}$ sparse random banded matrices, $b \in \RR^{n}$ random. The solution to this system is the transfer function for a time-delay system where entire state is the output (see standard references for time-delay
systems \cite{Gu:2003:STABILITY,Michiels2011,Michiels:2007:STABILITYBOOK}).

We replace line \ref{alg:Kinv} of Algorithm~\ref{alg:FIGMRES} with
\begin{align} \label{eq:z-pert}
	\tilde{z}_i = K_m^{-1} q_i + \Delta_i,
\end{align}
where $\Delta_i$ is random vector. The above introduces error to line \ref{alg:Kinv} of Algorithm~\ref{alg:FIGMRES} in a slightly different way than considered previously. Here the preconditioning matrix $K_m^{-1}$ is applied exactly but we introduce error with a random vector. The magnitude of the random vector $\Delta_i$ is determined in a way analogous to Proposition~\ref{prop1}. More precisely, we consider a bound on $p_i$ as in \eqref{eq:pj-ineq} where $p_i$ is the inner residual vector (see \eqref{eq:pj1}). We select $\ell_j = 1$, $\varepsilon = 10^{-10}$.

\begin{figure}[h]
	\includegraphics[scale=.5]{ran_pert_dir_solve.pdf}
	\caption{Convergence of Algorithm~\ref{alg:FIGMRES} for solving \eqref{eq:unshifted-trunc}, $m \rightarrow \infty$, $A(\mu)$ as in \eqref{eq:delay-A} with $n=961$, random perturbations as in \eqref{eq:z-pert}, $\norm{r_j}$ as in \eqref{eq:big-res}, $\ell_m = 1$, $\varepsilon = 10^{-10}$, $\varepsilon_{\text{inner}_j}$ (not plotted) corresponds to largest $\mu$, compare to direct solve on each iteration}
	\label{fig:asymfigs}
\end{figure}

\begin{figure}
	\begin{subfigure}[t]{0.6\columnwidth}
		\includegraphics[scale=.5]{rtilde1.pdf}
		\caption{Convergence $\norm{\tilde{r}_j}$, inner tolerance $\varepsilon_{\text{inner}_j}$ (not plotted) corresponds to each value of $\mu$ considered}
		\label{fig:rtilde}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.6\columnwidth}
		\includegraphics[scale=.5]{einner1.pdf}
		\caption{Iterations vs norm of $\varepsilon_{\text{inner}}$ as in \eqref{eq:pj-ineq}}
		\label{fig:einner}
	\end{subfigure}

	\begin{subfigure}[t]{0.6\columnwidth}
		\includegraphics[scale=.5]{r_rtilde.pdf}
		\caption{$\delta_j = \norm{r_j-\tilde{r}_j}$ as in \eqref{eq:distance}, $\delta_j \leq \varepsilon$ as predicted by Proposition~\ref{prop1}}
		\label{fig:r_rtilde}
	\end{subfigure}
	\caption{Convergence of Algorithm~\ref{alg:FIGMRES} for solving \eqref{eq:unshifted-trunc} with $m \rightarrow \infty$, $A(\mu)$ as in \eqref{eq:delay-A} with $n=961$, random perturbations as in \eqref{eq:z-pert}, $\norm{r_j}$ as in \eqref{eq:big-res}, $\norm{\tilde{r}_j}$ as in \eqref{eq:calc-r-tilde}, $\ell_j = 1$, $\varepsilon = 10^{-10}$}
	\label{fig:asymfigs2}
\end{figure}

\begin{figure}
	\begin{subfigure}[t]{0.6\columnwidth}
		\includegraphics[scale=.5]{sol_nep.pdf}
		\caption{Solutions $\lambda_i$ to the NEP \eqref{eq:NEP}}
		\label{fig:solnep}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.6\columnwidth}
		\includegraphics[scale=.5]{sol_eigs.pdf}
		\caption{Reciprocal solutions to the NEP \eqref{eq:NEP}, $\gamma_i = 1/\lambda_i$, i.e., eigenvalues of the $M_m K_m^{-1}$ as in \eqref{eq:MK-inv}}
		\label{fig:soleigs}
	\end{subfigure}
	\caption{$n=225$}
	\label{fig:background-conv}
\end{figure}

\begin{figure}
	\begin{subfigure}[t]{0.6\columnwidth}
		\includegraphics[scale=.5]{conv_plot2.pdf}
		\caption{$\mu=.025$}
		\label{fig:conv1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.6\columnwidth}
		\includegraphics[scale=.5]{conv_plot1.pdf}
		\caption{$\mu=.05$}
		\label{fig:conv2}
	\end{subfigure}
	\caption{Convergence of Algorithm~\ref{alg:FIGMRES} for solving \eqref{eq:unshifted-trunc} with $m \rightarrow \infty$, $A(\mu)$ as in \eqref{eq:delay-A} with $n=225$, random perturbations as in \eqref{eq:z-pert}, $\norm{r_j}$ as in \eqref{eq:big-res}, $\ell_m = 1$, $\varepsilon = 10^{-10}$, predicted convergence as in \eqref{eq:conv-bound} with $k=7$}
	\label{fig:convplots}
\end{figure}
In Figures~\ref{fig:asymfigs} and \ref{fig:asymfigs2} we illustrate the asymptotic convergence of our algorithm. Figure~\ref{fig:asymfigs} shows the convergence of Algorithm~\ref{alg:FIGMRES} applied to \eqref{eq:unshifted-trunc} with $m \rightarrow \infty$, $A(\mu)$ as in \eqref{eq:delay-A}. Here the algorithm is run one time for the largest value of $\mu$ and then the function handle $\tilde{x}_j(\mu)$ is evaluated for each of the smaller values of $\mu$ considered. As the algorithm is not run more than once, this corresponds to generating a new approximation without modifying the random perturbations. Thus, for a given choice of $\mu$, the random perturbations introduced into Algorithm~\ref{alg:FIGMRES} will not disrupt convergence for smaller values of $\mu$. As noted above, we can except very fast convergence for small values of $\mu$ as the residual of the underlying method vanishes quickly (see equation \eqref{eq:conv-bound}). The convergence of Algorithm~\ref{alg:FIGMRES} is displayed alongside the convergence of applying preconditioned GMRES to this problem, i.e., considering an exact solve with $A(0)$ on each iteration.

Figure~\ref{fig:rtilde} illustrates the convergence of the underlying method, i.e., $\norm{\tilde{r}_j}$ for the same values of $\mu$ as in Figure~\ref{fig:asymfigs} and Figure~\ref{fig:einner} shows the norm of $\varepsilon_{\text{inner}}$ as in \eqref{eq:pj-ineq} on each iteration for each value of $\mu$. It is clear that if we execute our algorithm one time for the largest value of $\mu$, we can reuse the inner stopping criteria for smaller choices of $\mu$, as the inner stopping criteria becomes less restrictive for smaller values of $\mu$. Figures~\ref{fig:rtilde} and \ref{fig:einner} together show the inverse relationship between the quantities $\tilde{r}_j$ and $\varepsilon_{\text{inner}}$ for a fixed value of $\varepsilon$, as described in equation \eqref{eq:inverse}. As predicted by the analysis above, the underlying method converges very fast for small values of $\mu$. As a result, a larger inner residual does not destroy convergence, leading to a faster algorithm.

Figure~\ref{fig:r_rtilde} shows the result of Proposition~\ref{prop1}, namely that the norm of the difference between the true residual and the residual of the underlying method is below $\varepsilon=10^{-10}$ on each iteration of Algorithm~\ref{alg:FIGMRES} if \eqref{eq:stop-crit} is fulfilled on each iteration.

Figure~\ref{fig:solnep} shows the solutions $\lambda_i$ to the polynomial eigenvalue problem given by
\begin{align} \label{eq:NEP}
	(-\lambda I + A_0 + A_1 e^{-\lambda})v = 0, v \neq 0
\end{align}
and Figure~\ref{fig:soleigs} shows the eigenvalues of the companion matrix $M_m K_m^{-1}$ as in \eqref{eq:MK-inv}, which correspond to the reciprocal solutions to \eqref{eq:NEP}, i.e., $\gamma_i = 1/\lambda_i$.

Figure~\ref{fig:convplots} illustrates the predicted convergence of Algorithm~\ref{alg:FIGMRES} as in \eqref{eq:conv-bound} along with the observed convergence for two different values of $\mu$. Here we have chosen $k=7$, as seen in Figure~\ref{fig:soleigs} and $\varepsilon = 10^{-10}$. The plots display observed convergence from applying the preconditioner inexactly (random perturbations as in \eqref{eq:z-pert}) and exactly (applying $A(0)^{-1}$ via direct solve). We observe convergence in fewer iterations for smaller values of $\mu$.


\begin{comment}
\textbf{Taylor series expansion for FOM}
If we alternatively consider FOM, then we can express $\norm{\tilde{r}_j}$ as follows.
\begin{align*}
	\norm{\tilde{r}_j} &= \norm{ e_1 \norm{c} - (I_j - \mu H_j) w_j} \\
	&= \norm{ e_1 \norm{c} - (I_j - \mu H_j) (e_1 \norm{c} + \mu H_j e_1 \norm{c} + \ldots)}
\end{align*}
since
\begin{align*}
	w_j &= (-\mu H_j + I_j)^{-1} (e_1 \norm{c}) \\
	&= e_1 \norm{c} + \mu H_j e_1 \norm{c} + \mu^2 H_j^2 e_1 \norm{c} + \ldots
\end{align*}
where $H_j$ and $I_j$ are square matrices of dimension $(j \times j)$. We see here that $\norm{\tilde{r}_j}$ goes to $0$ linearly in $\mu$.

In practice, Algorithm~\ref{alg:FIGMRES} converges in fewer iterations for smaller values of $\mu$.

The convergence bound in [our first paper] ???
Holds for 'pretty small' $\mu$ if we look at the residual of $A(\mu) x(\mu) = b$, i.e., the first $n$ entries of the GMRES solution. Not as well if we look at the residual to $(K-\mu M) v(\mu) = c$.
\end{comment}

\begin{comment}
\section{Iterative methods for inexact application of the preconditioner}
On iteration $i$ of Algorithm~\ref{alg:FIGMRES} applied to \eqref{eq:unshifted-trunc}, we compute $\tilde{z}_i$ for $i=1,\ldots,j$ as in \eqref{eq:flex-mult}, i.e., via an inexact application of the preconditioner. This amounts to an inexact application of $A_0^{-1}$. Within the framework of Algorithm~\ref{alg:FIGMRES}, the application of $A_0^{-1}$ by an iterative method can be performed to different tolerance levels on each iteration of the Arnoldi algorithm. The following analysis shows the decrease in complexity of Algorithm~\ref{alg:FIGMRES} over the standard preconditioned GMRES method.

If we assume $A_0 \in \CC^{n \times n}$ a general dense matrix, then the cost of applying $A_0^{-1}$ on $j$ iterations of the Arnoldi method via one LU factorization is
\[
	\mathcal{O} \big( \underbrace{2/3 n^3}_{\text{LU}} + \underbrace{jn^2}_{\text{Solve}} \big)
\]
since we must additionally solve 2 triangular systems on each Arnoldi iteration. If $A_0$ a sparse banded matrix with band of size $b$, then the cost of applying $A_0^{-1}$ on $j$ iterations of the Arnoldi method is reduced to
\[
	\mathcal{O} \big( \underbrace{nb^2}_{\text{LU}} + \underbrace{jnb}_{\text{Solve}} \big).
\]
In many applications, $A_0$ is a discretization of an elliptic partial differential equation. Applying $A_0^{-1}$ can be accomplished approximately with the standard GMRES method. That is, we use the method GMRES to solve a linear system on each iteration of the main GMRES algorithm, corresponding to applying the preconditioning matrix $K_m^{-1}$ inexactly.

The method GMRES tends to converge slowly for linear systems where the system matrix is as described above. Preconditioned GMRES offers improvement, however multigrid methods are optimal (see \cite{AxelVass1989,AxelVass1990,BMcR1984,CFHJM2000,DahEls1989} for literature on multigrid methods). \textbf{Did not finish listing the citations here.} We consider instead applying $A_0^{-1}$ approximately using a multigrid V-cycle on $j$ iterations of the Arnoldi method. The cost of this is thus reduced to
\[
	\mathcal{O} \big( jn \big)
\]
since multigrid methods have complexity $\mathcal{O}(n)$ for sparse systems of dimension $n \times n$. The cost is further reduced as the tolerance of the multigrid method is allowed to grow as the residual of the approximation decreases (see Section~\ref{sec:inner-tol}).
\end{comment}

\begin{comment}
\subsection{Low-rank variation}
Suppose now that $A(\mu) \in \CC^{n \times n}$ analytic and the higher order terms are of reduced rank, i.e.,
\begin{align}  \label{eq:A_reduced_rank}
    A(\mu) &= \sum_{i=0}^s A_i \mu^i + \sum_{i=s+1}^{\infty} \frac{1}{i!} U_i V^T \mu^i,
\end{align}
with $A_i$ as in \eqref{eq:Ai}, $U_i = U F^{(i)}(0) \in \CC^{n \times p}$, $U,V\in\CC^{n\times p}$, and $F^{(i)}(0) \in \CC^{p \times p}$.
\end{comment}

\subsection{Numerical PDE example}
We consider the numerical solution of
\begin{subequations} \label{helm}
\begin{alignat}{2}
	\left( \nabla^2 + \sin(\mu) k(x,y) + \cos(\mu) b(x,y) \right) u(x,y) &= f(x,y), \quad &&(x,y) \in \Omega \\
	u(x,y) &= 0, \quad &&(x,y) \in \partial \Omega
\end{alignat}
\end{subequations}
where
\begin{subequations}
\begin{eqnarray*}
k(x,y) &=& 10+10x \sin(\alpha \pi x y) \\
b(x,y) &=& \alpha \sin(2 \pi y^2)\\
f(x,y) &=& 500(x-1)^2 + 500y^2
\end{eqnarray*}
\end{subequations}
and $\Omega = [0,1] \times [0,1]$. We define a discretization $A_n(\mu) \in \mathbb{C}^{n^2 \times n^2}$ of \eqref{helm} as
\begin{align} \label{eq:disc1}
	A_n(\mu) := D_n + \sin(\mu) K_n + \cos(\mu) B_n,
\end{align}
where $D_n$ is defined by the standard 5-point stencil, i.e.,
\begin{align*}
	D_n := \frac{1}{h^2}
	\begin{bmatrix}
	D & -I & & \\
	-I & \ddots & \ddots & \\
	& \ddots & \ddots & -I \\
	& & -I & D
	\end{bmatrix} \in \mathbb{R}^{n^2 \times n^2}, \quad
	D =
	\begin{bmatrix}
	4 & -1 & & \\
	-1 & \ddots & \ddots & \\
	& \ddots & \ddots & -1\\
	& & -1 & 4
	\end{bmatrix} \in \mathbb{R}^{n \times n}
\end{align*}
with $h=1/(n+1)$ and
\begin{subequations}
\begin{eqnarray*}
	K_n &=& \text{diag} (\text{vec} (\hat{K}_n)) \in \mathbb{R}^{n^2 \times n^2} \\
	B_n &=& \text{diag} (\text{vec} (\hat{B}_n)) \in \mathbb{R}^{n^2 \times n^2},
\end{eqnarray*}
\end{subequations}
with
\[
	\hat{K}_n =
	\begin{bmatrix}
	k(x_1,y_1) & \cdots & k(x_1,y_n) \\
	\vdots & \ddots & \vdots \\
	k(x_n,y_1) & \cdots & k(x_n,y_n)
	\end{bmatrix}, \quad
	\hat{B}_n =
	\begin{bmatrix}
	b(x_1,y_1) & \cdots & b(x_1,y_n) \\
	\vdots & \ddots & \vdots \\
	b(x_n,y_1) & \cdots & b(x_n,y_n)
	\end{bmatrix},
\]
for $x_i=hi$, $i=1,\ldots,n$ and $y_j = hj$, $j=1,\ldots,n$. Similarly, we take
\[
	F_n = \text{diag} (\text{vec} (\hat{F}_n)) \in \mathbb{R}^{n^2 \times n^2},
\]
with
\[
	\hat{F}_n =
	\begin{bmatrix}
	f(x_1,y_1) & \cdots & f(x_1,y_n) \\
	\vdots & \ddots & \vdots \\
	f(x_n,y_1) & \cdots & f(x_n,y_n)
	\end{bmatrix}.
\]
Thus, we seek the solution $x_n(\mu) \in \mathbb{C}^{n^2}$ s.t.
\begin{align} \label{eq:num-ex1}
	A_n(\mu) x_n(\mu) = F_n.
\end{align}

\subsection{Numerical results, PDE example, Algorithm~\ref{alg:FIGMRES} with multigrid V-cycle with dynamic stopping criteria as inner solver}
\begin{figure}[h!]
\includegraphics[scale=.4]{fig1.pdf}
\caption{Convergence history for \eqref{eq:num-ex1}, $\mu=.8$, $n^2=3969$, $\kappa(A_n(\mu))=2.4136 \times 10^{3}$, multigrid V-cycle with dynamic inner stopping criteria as inner solver}
\label{fig:figure1}
\end{figure}

\begin{figure}[h!]
	\begin{subfigure}[t]{0.45\columnwidth}
		\includegraphics[scale=.40]{fig2.pdf}
		\caption{Dynamic inner stopping criteria according to \eqref{eq:pj-ineq}}
		\label{fig:figure2a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.45\columnwidth}
		\includegraphics[scale=.40]{fig2b.pdf}
		\caption{Fixed inner stopping criteria according to \eqref{eq:fixed-inner}}
		\label{fig:figure2b}
	\end{subfigure}
\caption{Convergence history for \eqref{eq:num-ex1}, $\mu=.8$, $n^2=3969$, $\kappa(A_n(\mu))=2.4136 \times 10^{3}$, $\varepsilon=10^{-10}$, $\ell_m=1$, multigrid V-cycle with dynamic stopping criteria as inner solver}
\label{fig:figure2}
\end{figure}

\begin{figure}[h!]
\includegraphics[scale=.5]{fig3.pdf}
\caption{$\mu=.8$, $n^2=3969$, $\kappa(A_n(\mu))=2.4136 \times 10^{3}$, $\ell_m = 1$, $\varepsilon = 10^{-10}$, multigrid V-cycle with dynamic stopping criteria as inner solver}
\label{fig:figure3}
\end{figure}

\textbf{Need larger simulations and change the code you are using in the multigrid algorithm.}

Here the inner solver is a multigrid V-cycle where the tolerance is chosen dynamically as described in Section~\ref{sec:inner-tol}. In Figure~\ref{fig:figure1} we plot the convergence history (norm of the true residual) of Algorithm~\ref{alg:FIGMRES} along with the norm of the variable inner stopping tolerance $\varepsilon_{\text{inner}}$ as in \eqref{eq:pj} with $\ell_m = 1$ and $\varepsilon = 10^{-10}$. We see that the algorithm returns a small residual $r_m$ even with an inner stopping tolerance which increases on each iteration of the outer loop.

Figure~\ref{fig:figure2} shows the convergence history as a function of CPU time. Figure~\ref{fig:figure2a} shows the variable inner stopping tolerance as in \eqref{eq:pj-ineq}. In Figure~\ref{fig:figure2b} we consider instead a constant inner stopping tolerance, that is,
\begin{align} \label{eq:fixed-inner}
	\norm{p_j} \leq \varepsilon,
\end{align}
with $\varepsilon = 10^{-10}$.

Figure~\ref{fig:figure3} shows a plot of the numerical solution.

\section{Conclusions and outlook}
\textbf{Need to write.}

\section{Acknowledgements}
\textbf{Need to write.}

\bibliographystyle{plain}
\bibliography{siobhanbib,eliasbib}

